Deep Non-Rigid Structure from Motion

Current non-rigid structure from motion (NRSfM) algorithms are mainly limited with respect to: (i) the number of images, and (ii) the type of shape variability they can handle. This has hampered the practical utility of NRSfM for many applications within vision. In this paper we propose a novel deep neural network to recover camera poses and 3D points solely from an ensemble of 2D image coordinates. The proposed neural network is mathematically interpretable as a multi-layer block sparse dictionary learning problem, and can handle problems of unprecedented scale and shape complexity. Extensive experiments demonstrate the impressive performance of our approach where we exhibit superior precision and robustness against all available state-of-the-art works in the order of magnitude. We further propose a quality measure (based on the network weights) which circumvents the need for 3D ground-truth to ascertain the confidence we have in the reconstruction.

==> recover_mocap.table.tex <==
\begin{table}[t]
 \centering
 \footnotesize
 \begin{tabular}{C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}}
  \specialrule{0.8pt}{1pt}{1pt}
             & PMP   & Alternate & Convex         & Ours           \\
  \hline
  Subject 13 & 0.390 & 0.293     & 0.259          & \textbf{0.229} \\
  Subject 14 & 0.393 & 0.308     & \textbf{0.258} & 0.261          \\
  Subject 15 & 0.340 & 0.286     & 0.204          & \textbf{0.200} \\
  \specialrule{0.8pt}{1pt}{1pt}
 \end{tabular}
 \caption{Comparison of our method against the state-of-the-art algorithms in
  single image human pose estimation task. Our method achieves competitive
  results using solely 2D projections while all others learn from
  3D ground truth.}
 \label{tab:recover}
\end{table}


==> teaser.image.tex <==
\begin{figure}[t]
 \centering
 \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=0.24\linewidth]{figures/teaser_01_01774.png}
  \includegraphics[width=0.24\linewidth]{figures/teaser_23_01320.png}
  \includegraphics[width=0.24\linewidth]{figures/teaser_64_01188.png}
  \includegraphics[width=0.24\linewidth]{figures/teaser_102_00450.png}
  \caption{Non-rigid object: moving person.}
 \end{subfigure}

 \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=0.24\linewidth]{figures/teaser_chair_05.png}
  \includegraphics[width=0.24\linewidth]{figures/teaser_chair_18.png}
  \includegraphics[width=0.24\linewidth]{figures/teaser_chair_15.png}
  \includegraphics[width=0.24\linewidth]{figures/teaser_chair_22.png}
  \caption{Object category: chair.}
 \end{subfigure}

 \caption{Randomly selected 3D reconstructions by our deep \nrsfm method based
  on multi-layer sparse coding model.
  Spheres in (a) and red cubes in (b) are reconstructed points. Bars, planes
  are manually added for visualization.}
 \label{fig:teaser}
\end{figure}

